A Unified Feature Representation for Lexical Connotations

Ideological attitudes and stance are often expressed through subtle meanings of words and phrases. Understanding these connotations is critical to recognizing the cultural and emotional perspectives of the speaker. In this paper, we use distant labeling to create a new lexical resource representing connotation aspects for nouns and adjectives. Our analysis shows that it aligns well with human judgments. Additionally, we present a method for creating lexical representations that captures connotations within the embedding space and show that using the embeddings provides a statistically significant improvement on the task of stance detection when data is limited.

==> tables/multi_ex.tex <==
\begin{table}[t]
\centering
\vspace{-33pt}
\begin{tabular}{ll}
\hline
\textbf{English: goat} & \multicolumn{1}{c}{\textbf{Russian: \begin{otherlanguage*}{russian}козёл\end{otherlanguage*} (kozyol)}} \\ \hline \hline
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\textbullet \  mammal\\ \textbullet \ \textit{(slang)}\\ \quad lecherous man\\ \textbullet \ scapegoat\\ \textbullet \  \textit{(slang)} a Pontiac \\ \quad GTO car\\ \hfill\end{tabular}} & 
\begin{tabular}[c]{@{}l@{}}\textbullet \  he-goat or scapegoat\\ \textbullet \  \textit{(slang, derogatory)} \\ \quad idiot, jerk, ass\\ \textbullet \  \textit{(slang, very offensive)} \\ \quad prison informer\\ \textbullet \ \textit{(slang, very offensive)} \\ \quad homosexual\end{tabular} \\ \hline
\end{tabular}
\caption{Connotation in the first definitions from Wikitionary for ``goat'' and its Russian translation.}\label{tab:defex}
\end{table}

==> tables/stance_stats.tex <==
\begin{table}[t]
\centering
\begin{tabular}{l|c}
    \hline
    % \# topics & 16 \\
    \# \textit{L} topics (${>}7k$ ex each) & 4 \\
    \# \textit{M} topics (${\sim}2k$ ex each) & 5\\
    \# \textit{S} topics ($30$-$300$ ex each) & 7\\
    % \# ex & ${\sim}59k$\\
    \hline
\end{tabular}
\caption{Topic Statistics for the stance data.}
\label{tab:stancedata}
\end{table}
